Cooperation risk and Nash equilibrium: quantitative description for realistic players

The emergence of cooperation figures among the main goal of game theory in competitive-cooperative environments. Potential games have long been hinted as viable alternatives to study realistic player behavior. Here, we expand the potential games approach by taking into account the inherent risks of cooperation. We show the Public Goods game reduce to a Hamiltonian with one-body operators, with the correct Nash Equilibrium as the ground state. The inclusion of punishments to the Public Goods game reduces the cooperation risk, creating two-body interaction with a rich phase diagram, where phase transitions segregates the cooperative from competitive regimes.

==> prisoner.tex <==
\section{Prisoner Dilemma}
\label{sec:prisoner}


The Prisoner Dilemma (PD) is a classic cooperative-competitive problem
in Game Theory which dwells about player decisions and their
outcomes. In its simplest formulation with two players, each player
may either cooperate or defect. Mutual cooperation results in a reward
$R$ whereas mutual defection produces punishment $P$. In addition, one
player may defect while the other cooperates. In this case, the
defector earns a temptation reward $T$ and the cooperator loses $S$
(sucker price). The PD depends on the relationship between these
variables, namely, $T > R > P > S$ and $2 R > T+S$.

One way to summarize the PD employs the
payoff matrix $E$. Following \cite{hauertEcoLett2005}, let $P=0$,
$S=-c$,  $T = b$ and $R=b-c$ with $b  \geq 0$ and $c\geq 0$ so that
the payoff matrix reads    
\begin{equation}
E = \left(\begin{array}{cc}
b-c & -c\\
b & 0
\end{array}\right).
\label{eq:e}
\end{equation}
Although the formulation in Eq.~(\ref{eq:e}) enjoys ample usage, we
stress it is just a compact way to store the outcomes in the
PD. However, it is inconvenient to represent global properties of
the system since it only considers the payoffs for a single player.   
% One way to overcome this issue considers the payoffs from both
% players, in which case we map the available strategies of each PD player
% (cooperator, defector) as a two-level system ($\uparrow$,
% $\downarrow$).  Thus, in the base $\lvert \uparrow\uparrow \rangle$, 
% $\lvert\uparrow\downarrow \rangle$, $\lvert \downarrow\uparrow
% \rangle$ and $\lvert \downarrow\downarrow \rangle$,
% the complete payoff matrix reads
One way to overcome this issue considers the payoffs from both
players, in which case we map the available strategies of each PD player
(cooperator, defector) as a two-level system ($1$, $0$),
respectively. Thus, in the base $\lvert 1 1 \rangle$, $\lvert 1 0
\rangle$, $\lvert 0 1 \rangle$ and $\lvert 0 0 \rangle$, the complete
payoff matrix reads 
\begin{equation}
  E =
\Delta
  \left(\begin{array}{cccc}
2&&&\\
&1&&\\
&&1&\\
&&&0
\end{array}\right),
\label{eq:e2}
\end{equation}
where $\Delta = b - c$. We emphasize $E$ is not necessarily a diagonal
matrix for general relationships between $R,T,S$ and $P$
\cite{szaboPhysRep2016}. 

 
Next, we recover the Hamiltonian operator $\hat{H}$ of the
system -- hereafter, operators are identified by the hat symbol. 
In dynamical systems, $\hat{H}$ extracts global properties of
configurations, usually the total energy, and dictates the time
evolution of the system. More specifically, the matrix representation
of $\hat{H}$ must be equal to $-E$ as players tend to favor  earnings
in the absence of risks. 
% We proceed by recovering an effective Hamiltonian $\hat{H}$ whose
% matrix representation must equal $-E$ in Eq.~({\ref{eq:e2}}). The
% negative signal remind us that players ultimately favor earnings in
% the absence of risks.
As starting point, we assume $\hat{H}$ can be broken down as the
summation of individual payoffs, $\hat{H}\equiv
\hat{\varepsilon}_0+\hat{\varepsilon}_1$, which leaves us with the
task of finding the exact expression for
$\hat{\varepsilon}_{0,1}$. For that purpose, let us define the number 
operator $\hat{n}_k$ to measure the strategy of the $k$-th
player, \textit{i.e.}, $\hat{n}_0\lvert n_0n_1\rangle = n_0\lvert n_0
n_1\rangle $ and $\hat{n}_1\lvert n_0n_1\rangle = n_1\lvert n_0
n_1\rangle $. Since each $\hat{n}_k$ span a $2$-level basis, with
eigenvalue $1$ ($0$) associated with $\lvert 1 \rangle$ ($\lvert 0
\rangle$), the 
operators $\hat{n}_k$ form suitable building blocks for
$\hat{\varepsilon}_{0,1}$. In fact, consider the most general payoff
operator for player $k=0$, namely, $\hat{\varepsilon}_0 =  a_{11}
\hat{n}_0\hat{n}_1 + a_{10} \hat{n}_0(1-\hat{n}_1) +a_{01}
(1-\hat{n}_0)\hat{n}_1+ a_{00} (1-\hat{n}_0)(1-\hat{n}_1)$. Here, the 
action of $\hat{n}_0\hat{n}_1$ produces non-vanishing values if both
players cooperate, $\hat{n}_0(1- \hat{n}_1)$ results in non-vanishing
output if player $k=0$ cooperates but $k=1$ defects,
\textit{etc}. An analogous expression is derived for
$\hat{\varepsilon}_1$. From Eq.~(\ref{eq:e}), one  quickly realizes
$a_{11}=b-c$, $a_{10}=-c$, $a_{01}=b$ and $a_{00}=0$  so that
\begin{subequations}
  \begin{align}
    \hat{\varepsilon}_0 = &  b \hat{n}_1 - c \hat{n}_0  ,\\
    \hat{\varepsilon}_1 = &  b \hat{n}_0 - c \hat{n}_1.
  \end{align}
\end{subequations}
These results imply that products between number operators, also known
as two-body operators, cancel out during the evaluation of individual 
payoffs. As a consequence, the two-player Hamiltonian reads
\begin{equation}
\hat{H} =-\Delta \left(\hat{n}_0+\hat{n}_1\right),
\label{eq:h_ini}
\end{equation}
which only supports one-body interactions. Eq.~(\ref{eq:h_ini})
is equivalent to a paramagnetic spin system under the action
of the magnetic field $h=\Delta/2$. Accordingly, cooperation becomes
more prominent for 
increasing  $\Delta$. At $\Delta = 0$, the system exhibits $Z_2$
symmetry ($1/2$-spin inversion), producing equal cooperation and
defection rates.

The existence of $\hat{H}$ leads to the formulation of the PD as a
potential game \cite{szaboPhysRep2016}. However, even though $\hat{H}$
describes players' payoffs, Eq.~(\ref{eq:h_ini}) favors cooperation as
long as $\Delta > 0$, incompatible with the expected behavior of NE.
Therefore, $\hat{H}$ requires further corrections to take into
account the inherent risks associated with cooperation.

Luckily, the NE condition can also be used to model the risk. The
condition states the NE occurs whenever a  player cannot improve its
own earnings by changing its current 
strategy, regardless of the strategies of the remaining players. We
also note that the NE condition implicitly assumes the various player 
strategies are uncorrelated, to accommodate the assumption of independent
strategy variations. Let $ \langle \varepsilon_0\rangle =  b
\langle n_1\rangle - c \langle n_0 \rangle$ be the average earnings of
player $k=0$ in a  single round PD game with two players, with
$\langle n_{0,1}\rangle \in [0,1]$.  The NE condition reads  $\partial
\langle \varepsilon_0\rangle/\partial \langle n_0 \rangle =  -c $,
stating that increasing cooperation incurs into additional costs or
damages, with an analogous result for the other player. Thus, the
addition of linear operators $\hat{n}_{0,1}$ with coupling
constants $\mu=c$ produce the desired PD Hamiltonian: 
\begin{equation}
\hat{H} =-{\Delta'}
\left( 
\hat{n}_0 +\hat{n}_1
\right),
\label{eq:h}
\end{equation}
where $\Delta' = \Delta - c$.
The behavior of the state with the lowest eigenvalue of $\hat{H}$
(ground state) also merits further discussion, as it asserts whether
players favor individual benefits over losses or \textit{vice versa}.  
It is worth noting that even though
$\Delta > 0$ in the PD, the coupling $\Delta'$ might acquire negative
values, in which case the PD becomes an antiparamagnetic spin system.
Therefore, the ground state with $b > 2 c$ holds only
collaborators, whereas for $ b < 2 c$, the ground state
reproduce the strategy profile in which every player is a defector, 
consistent with the expected Nash equilibrium.


The generalization for $N$ simultaneous games among $N$ players is
straightforward:
\begin{align}
  \label{eq:hk}
  \hat{H} & = -\Delta'\sum_{k=0}^{N-1}q_{k} \hat{n}_{k},
\end{align}
in which the coordination number $q_k = \sum_{\ell=0}^{N-1}A_{\ell
  k}$, evaluated from the $N\times N$ adjacency matrix $A$
\cite{albertRevModPhys2002, szaboPhysRep2007}, maps player
interactions through  various games. Again, $c > \Delta$ inhibits
cooperation but the effective risk for the $k$-th player is increased
$q_k$ times as a consequence of participation in multiple games. The
corresponding ground state $\lvert 0 0 \cdots 0\rangle$ reflects
the expected Nash equilibrium for rational players. However, games
formed exclusively by rational players are unlikely to occur under
normal circumstances. Instead, players may select sub-optimal
strategies, resulting in a ground state that differs from the expected
NE, even for $c > \Delta$. 

To model the sub-optimal strategy selection, one introduces a scale
$\beta\in \mathbb{R}^+$, where 
$\beta=0$ ( $\beta \rightarrow\infty$) refers to random (optimal)
strategy
\cite{blume1993,szaboPhysRep2016,szaboPhysRevE2014,szaboPhysRevE2015}.
The actual value of $\beta$ takes into consideration a 
number of factors, including general player behavior, reward's
relevance and availability, \textit{etc}. Furthermore, the parameter
$\beta$ should be a representative value for a large pool of players,
much larger than $N$. Under these circumstances, we may establish a formal
connection between Game Theory and Statistical Physics, in which
$\beta$ plays the role of inverse temperature of a thermal reservoir
\cite{reichl1998}. As a result, the likelihood of the NE increases with
vanishing temperatures for $c > \Delta$. Several other properties are
derived from the partition function $Z(\beta)\equiv Z $. For instance,
average strategy per player $\langle n \rangle = (1/2)[1+\tanh(\beta\Delta'
)]$,  in the one-dimensional chain with periodic boundary conditions
(see Fig.~\ref{fig:prisoner_numerical}). 


\begin{figure}
  \includegraphics[width=0.95\columnwidth]{sample10000.eps}
  \caption{\label{fig:prisoner_numerical}
    Average strategy in the Prisoner's Dilemma for three different ratios
    $c/b$.  $N=100$ players take part in the game, each with
    coordination number $q = 2$. Shaded regions correspond to the standard
    error. At $b = 2 c$, the density of cooperators equal the density
    defectors. Cooperation becomes the dominant strategy for $c/b <
    1/2$ for rational players ($\beta > 0$).} 
\end{figure}



The absence of correlation among player strategies is another striking
feature in Eq.~(\ref{eq:hk}), due to the lacking of player-player
interactions. 
% For instance, in our toy model Eq.~(\ref{eq:hN}), 
% $\langle \sigma_k \sigma_j \rangle  - \langle \sigma_k\rangle\langle
% \sigma_j\rangle=0$, which holds for any symmetric adjacency matrix
% $A$ and $k\neq j$.
Indeed, the emergence of collective phenomena among $N$ players, and
hence correlations, demands
two-body or higher operators to offset contributions from one-body
operators \cite{cardy, henkel}. Based on well-known examples of
Statistical Physics -- for instance, Ising and XXZ models
\cite{amit2005,kogut, alcarazAnnPhys1994}  -- the competition between
the symmetries of one- and two-body operators allows for richer phase
diagrams concerning the strategy profiles of $N$ players.

% In what follows, we address the Public Goods game and introduce
% punishment and extra rewards to show how two-body operators affects the
% general properties of player strategies.

 


%% Given the results listed so far, it has become clear the
%% Hamiltoni an of Eq.~(\ref{eq:hN}) does not recovers the Ising model. Therefore, we \sout{can only but} refute the PD
%% Hamiltonian proposed by Adami and Hintze and their conclusions
%% regarding cooperation in the PD. We base our reasoning in what
%% follows.  



%% First, the PD Hamiltonian put forward in Ref.~\cite{adami2017} relies
%% entirely in the periodicity of the model: homogeneous interactions and
%% periodic boundary condition (PBC) alike. Since their PD Hamiltonian
%% commutes with both forward- and backward-translations, configurations
%% related by translations produce the same energy. In practice, the
%% translation symmetry implies that the total energy evaluated using the
%% single player payoff matrix or $(E+E^{\dag})/2$ produce the same
%% values. However, the later procedure cancels exactly every
%% contribution from two-body operators.  To decide whether the model
%% should be Ising or paramagnetic, it is sufficient to lift the PBC. As
%% evidence, consider the configurations  $\lvert c_1\rangle =\lvert
%% \uparrow\downarrow\downarrow\rangle$ and  $\lvert c_2\rangle =\lvert
%% \downarrow\downarrow\uparrow\rangle$ under  the action of the PD
%% Hamiltonian in Ref.~\cite{adami2017}. For PBC, their energies
%% $e_1=e_2=\Delta$ are equal since $\lvert c_2\rangle$ is related by
%% $\vert c_1\rangle$ by a translation. However, for open boundary
%% conditions (OBC), $e_1=b$ and $e_2=-c$ even though both configurations
%% hold a pair of players with equal strategy and a pair with differing
%% strategy, which is \emph{incompatible} with 1D Ising model -- with or
%% without a homogeneous magnetic field. Therefore, we can safely refute
%% the Ising model for OBC and PBC. 

%% Second, in Ref.~\cite{adami2017}, the Authors considered $\alpha =1$ to
%% construct their PD Hamiltonian. This particular choice favors
%% configurations that hold more defectors than collaborators, as
%% collaboration always produce a positive net energy for the system in
%% the PD. Hence, their conclusion about emergence of collaboration in
%% the PD depends on the correctness of their assumption about the
%% maximization of costs over benefits, which seems rather
%% counter-intuitive. Indeed, thermodynamical arguments reinforce the
%% choice $\alpha < 0$ but still lack proper foundations within Game
%% Theory. This is arguably the most problematic issue as it requires
%% additional individual information about player behavior, which may
%% break translational symmetry or even change over time. 















==> public_single.tex <==
\section{Public Goods}
\label{sec:public}

The operatorial formulation and results from Sec.~\ref{sec:prisoner}
can be generalized to the Public Goods (PG) games. The rules are
straightforward. 
Players may forfeit the cost $c$ from their own assets to a public
resource (collaborator), or keep $c$ (defector). The public resource is
then increased by the factor $b/c$ and, afterward, redistributed
equally among all players. Since players still receive their share
regardless of their own contributions, defectors lower the returns of
collaborators while increasing their own earnings, thus establishing
the cooperative-competitive scenario.   

\begin{figure}[htb]
  \includegraphics[width=0.4\columnwidth]{players.eps}
  \caption{\label{fig:publicplayers} Public goods (PG)
    game with $N$ players. Each player is assigned an unique
    identifier $k=0,1,\ldots,N-1$. Collaborators (blue) increase the
    size of public resource by bearing the entry cost $c$ and then
    receive their shares in return (bi-directional arrow). Defector
    (red) keep their assets but still receive share (one-directional
    arrow). }   
\end{figure} 

Following Sec.~\ref{sec:prisoner}, we map individual player strategies
(cooperator, defector) into a two-level system ($\lvert 1 \rangle,
\lvert 0 \rangle$). In this section, $N$ players partake in a single
PG game, with a single resource pool (see
Fig.~\ref{fig:publicplayers}). The neighborhood is described by 
the adjacency matrix $A$, with matrix elements $A_{ij} = 1-
\delta_{ij}$. Each player is labeled by a unique identifier $k=0, 1,
\ldots, N-1$, with coordination number $q_k=\sum_j A_{j k} = N -1$. 


As in the PD, we must evaluate the operator $\hat{\varepsilon}_k$
concerning individual payoff of $k$-th player. Individual payoffs are
simply the summation of earnings derived from cooperative strategies
with defective strategies, which are respectively,
\begin{subequations}
\begin{align}
  \hat{\Pi}^C_k = 
  & \left[ \frac{b}{N}
    \sum_{\ell=0}^{N-1}\hat{n}_{\ell}
    - c\, \hat{n}_{k} 
    \right]\hat{n}_k ,    \label{eq:pi_c}
  \\
  \hat{\Pi}^D_k =
  &\left[ \frac{b}{N}
    \sum_{\ell=0}^{N-1}\hat{n}_{\ell}
    - c\, \hat{n}_{k} 
    \right](1-\hat{n}_k).
  \label{eq:pi_d}
\end{align}
\end{subequations} 
The operator inside square brackets in Eqs.~(\ref{eq:pi_c}) and
(\ref{eq:pi_d}) subtracts the cost $c$ whether player $k$ paid or not
from his share. The summation of Eqs.~(\ref{eq:pi_c}) with
(\ref{eq:pi_d}) produces
\begin{equation}
  \hat{\varepsilon}_k= \frac{b}{N}\sum_{\ell = 0}^{N-1}\hat{n}_{\ell}
  - c\, \hat{n}_{k},
  \label{eq:earnings_pg}
\end{equation}
which holds only one-body operators. From Eq.~(\ref{eq:earnings_pg})
we evaluate the cooperation risk $\mu_k =-{\partial \langle
  \varepsilon_k \rangle}/{\partial\langle  n_k\rangle} = c -
{b}/{N}$. 
% \begin{equation}
%   \mu_k=-\frac{\partial \langle \varepsilon_k \rangle}{\partial\langle
%     n_k\rangle}=c - \frac{b}{N}.
% \end{equation}
As expected, the cooperation risk exhibits translational invariance,
$\mu_k\equiv \mu$, and equals to the  amount invested minus the
minimum returns. 


% The PG Hamiltonian, with players aiming for increasing returns but
% avoiding risks, is
% \begin{subequations}
% \begin{align}
%   \hat{H} &=-
%   \sum_{k=0}^{N-1}\left( h_k - \mu_k    \right)\hat{n}_k,
%   \label{eq:pg} \\
%   {h_k} & = b\left(\frac{1+\theta q_k}{1+q_k}\right)+
%           b\sum_{rs=0}^{N-1}\frac{A_{kr}(\delta_{rs}+\theta 
%           A_{rs})}{1+q_r}-c(1+\theta q_k).
% \end{align}
% \end{subequations}

Players in PG game aim for increasing returns while avoiding
risks, and are described by the PG Hamiltonian 
\begin{equation}
\hat{H}= -\sum_{k=0}^{N-1}\left(\hat{\varepsilon}_k + \mu_k\hat{n}_{k}
\right)  =-\sum_{ k=0}^{N-1}( \Delta-\mu)\hat{n}_{k},
\label{eq:h_pg}
\end{equation}
 with $\mu =c - b/N$. Similar to the PD, the two-body contributions in
 Eqs.~(\ref{eq:pi_c}) and (\ref{eq:pi_d}) cancel out  and the problem
 reduces either into a paramagnetic or antiparamagnetic system,
 depending on the difference between $\Delta$ and $\mu$. As a result,
 $\hat{H}$ fails to produce correlation among players. This property 
is a direct consequence of symmetric returns in the PG. 



With Eq.~(\ref{eq:h_pg}) in hands, the partition function is $Z_0
=\prod_{k} \left[1+\textrm{e}^{\beta (\Delta-\mu)} \right]$, so that the
average cooperation rate becomes 
\begin{equation}
  \langle n_k\rangle\equiv \bar{n} = \frac{1}{1+ \textrm{e}^{-\beta(\Delta-\mu)}}.
\end{equation}
Hence,  $\Delta  > \mu$ favors cooperation for large values of
$\beta$. Conversely,  $\Delta  < \mu$  inhibits cooperation as the
player becomes aware of risks. More importantly, $\langle n_jn_k\rangle
-\langle n_j\rangle \langle n_k\rangle = 0$ so there is no correlation
between players' strategies.




